Slicing Unbalanced Optimal Transport

Optimal transport (OT) is a powerful framework to compare probability measures, a fundamental task in many statistical and machine learning problems. Substantial advances have been made in designing OT variants which are either computationally and statistically more efficient or robust. Among them, sliced OT distances have been extensively used to mitigate optimal transport's cubic algorithmic complexity and curse of dimensionality. In parallel, unbalanced OT was designed to allow comparisons of more general positive measures, while being more robust to outliers. In this paper, we bridge the gap between those two concepts and develop a general framework for efficiently comparing positive measures. We notably formulate two different versions of sliced unbalanced OT, and study the associated topology and statistical properties. We then develop a GPU-friendly Frank-Wolfe like algorithm to compute the corresponding loss functions, and show that the resulting methodology is modular as it encompasses and extends prior related work. We finally conduct an empirical analysis of our loss functions and methodology on both synthetic and real datasets, to illustrate their computational efficiency, relevance and applicability to real-world scenarios including geophysical data.

==> sections/sec_theory.tex <==
\section{Sliced Unbalanced OT and Unbalanced Sliced OT: Theoretical Analysis}
\label{sec:theory}
We propose two strategies to make unbalanced OT scalable by leveraging sliced OT. This yields two novel loss functions, defined below.

\begin{definition} \label{def:suot_usot}
    Let $\al, \be \in \Mmp(\Rd)$ \cb{and $\varphi_1, \varphi_2$ two entropy functions}. The \textbf{Sliced Unbalanced OT} loss ($\SUOT$) and the \textbf{Unbalanced Sliced OT} loss ($\RSOT$) between $(\al,\be)$ are defined as, 
    \begin{align}
        \SUOT(\al, \be) &\triangleq \int_{\sphereD} \UOT(\thsss\al, \thsss\be) \rmd \unifS(\theta) \,, \label{eq:suot_primal} \\
        \RSOT(\al, \be) &\triangleq \inf_{(\pi_1,\pi_2)\in\Mmp(\Rd)^2} \SOT(\pi_1,\pi_2)%
        + \rmD_{\varphi_1}(\pi_1|\alpha) + \rmD_{\varphi_2}(\pi_2|\beta) \, .\label{eq:def-rsot}
    \end{align}
\end{definition}

$\SUOT(\al, \be)$ compares $\al$ and $\be$ by solving the UOT problem between $\thsss \al$ and $\thsss \be$ for $\theta \sim \unifS$. Note that SUOT extends the sliced partial OT problem \citep{bonneel2019spot,bai2022sliced} (where $\D_{\phi_i}=\rho_i\TV$) by allowing the use of arbitrary $\varphi$-divergences. On the other hand, USOT is a completely novel approach and stems from $\UOT(\al, \be) = \inf_{(\pi_1,\pi_2)\in\Mmp(\Rd) \times \Mmp(\Rd)}   \OT(\pi_1,\pi_2) + \rmD_{\varphi_1}(\pi_1|\alpha) + \rmD_{\varphi_2}(\pi_2|\beta)$. %


\begin{figure*}[!t]
  \centering
  \includegraphics[width=.9\textwidth]{figures/intro_RSOT.png}
  \caption{{\bf Toy illustration} on the behaviors of $\SUOT$ and $\RSOT$. {\em (left)} Original 2D samples and slices used for illustration. KDE density estimations of the projected samples: {\color{Gray} grey}, original distributions, {\color{Rhodamine} colored}, distributions reweighed by $\SUOT$  {\em (center)}, and reweighed by $\RSOT$ {\em (right)}.
  }
  \label{fig:intro}
\end{figure*}
\textbf{$\SUOT$ vs. $\RSOT$.} SUOT and USOT differ in how the transportation problem is penalized: $\SUOT(\al, \be)$ regularizes the marginals of $\pi_\theta$ for $\theta \sim \unifS$ where $\pi_\theta$ denotes the solution of $\UOT(\thsss \al, \thsss \be)$, while $\RSOT(\al, \be)$ operates a geometric normalization directly on $(\al, \be)$. We illustrate this difference on the following practical setting: we consider $\al,\be\in\Mmp(\rset^2)$ where $\al$ is polluted with some outliers, and we compute $\SUOT(\al, \be)$ and $\RSOT(\al, \be)$. We plot the input measures and the sampled projections $\{\theta_k\}_k$ (\Cref{fig:intro}, left), the marginals of $\pi_{\theta_k}$ for $\SUOT$ and the marginals of $(\theta_k^\star)_\sharp \pi$ for $\RSOT$ (\Cref{fig:intro}, right). 
As expected, $\SUOT$ marginals change for each $\theta_k$.
We also observe that the source outliers have successfully been removed for any $\theta$ when using $\RSOT$, while they may still appear with $\SUOT$ (e.g. for $\theta=120^\circ$): this is a direct consequence of the penalization terms $\D_{\phi_i}$ in $\RSOT$, which operate on $(\al, \be)$ rather than on their projections.

\textbf{Theoretical analysis.} In the rest of this section, we study the theoretical properties of $\SUOT$ and $\RSOT$. All proofs are provided in \Cref{app:proof-misc}. 
We first identify the conditions on the cost $\Co$ and entropies $\varphi_1, \varphi_2$ under which the infimum is attained in $\UOT(\thsss \al, \thsss \be)$ for $\theta \in \sphereD$ and in $\RSOT(\al, \be)$. %
\cb{
\begin{proposition}{\textbf{(Existence of minimizers)}}
\label{prop:exist-minimizer}
    Assume that $\Co$ is lower-semicontinuous and that either (i) $\phi_{1,\infty}^\prime=\phi_{2,\infty}^\prime=+\infty$, or (ii) $\Co$ has compact sublevels on $\rset \times \rset$ and $\phi_{1,\infty}^\prime+\phi_{2,\infty}^\prime +\inf \Co >0$.
    Then the solution of $\SUOT(\al,\be)$ and $\RSOT(\al,\be)$ exist, %
    \ie~the infimum in \eqref{eq:suot_primal} and \eqref{eq:def-rsot} is attained.
    More precisely, there exists $(\pi_1,\pi_2)$ which attains the infimum for $\RSOT(\al,\be)$ (see~\Eqref{eq:def-rsot}).
    Concerning $\SUOT(\al,\be)$, there exists for any $\theta\in\supp(\unifS)$ a plan $\pi_\theta$ attaining the infimum in $\UOT(\thsss\al,\thsss\be)$ (see~\Eqref{eq:primal-uot}).
\end{proposition}
}
\cb{In particular, the assumptions are met for the settings of interest $\D_{\varphi_1}=\D_{\varphi_2}=\KL$ since $\varphi_\infty' = +\infty$, or $\D_{\varphi_1}=\D_{\varphi_2}=\TV$ and $C_1(x,y) = |x-y|^p$ since $\varphi_\infty'=1$ \citep[Section 2.1]{sejourne2022unbalanced}.}

We also show that these optimization problems are convex, both $\SUOT$ and $\RSOT$ are jointly convex w.r.t. their input measures, and strong duality holds (\Cref{thm:duality-rsot}). Next, we prove that $\SUOT$ and $\RSOT$ have similar topological properties as $\UOT$, e.g., metric axioms.
\begin{proposition}{\textbf{(Metric properties)}} \label{prop:metric-suot}
    \emph{(i)} Suppose $\UOT$ is non-negative, symmetric and/or definite on $\Mmp(\rset) \times \Mmp(\rset)$. Then, $\SUOT$ is respectively non-negative, symmetric and/or definite on $\Mmp(\Rd) \times \Mmp(\Rd)$. If there exists $p \in [1, +\infty)$ s.t. for any $\al,\be,\ga\in\Mmp(\rset)$, $\UOT^{1/p}(\al,\be)\leq \UOT^{1/p}(\al,\ga) + \UOT^{1/p}(\ga,\be)$, then $\SUOT^{1/p}(\al,\be)\leq \SUOT^{1/p}(\al,\ga) + \SUOT^{1/p}(\ga,\be)$.

    \emph{(ii)} For any $\al, \be \in \Mmp(\Rd)$, $\RSOT(\al, \be) \geq 0$. If $\varphi_1=\varphi_2$, $\RSOT$ is symmetric. If $\D_{\varphi_1}$ and $\D_{\varphi_2}$ are definite, then $\RSOT$ is definite. If $\Co(x,y)=\abs{x-y}$ and $\D_{\varphi_1}=\D_{\varphi_2}=\rho\TV$, then, $\RSOT$ satisfies the triangle inequality. 
\end{proposition}

By \Cref{prop:metric-suot} (i), establishing the metric axioms of $\UOT$ between \emph{univariate} measures (e.g., as detailed in \cite[Section 3.3.1]{sejourne2022unbalanced}) suffices to prove the metric axioms of $\SUOT$ between \emph{multivariate} measures.
For example, since GHK is a metric for $p=2$ \citep{liero2018optimal}%
, so is the induced $\SUOT$.

In our next theorem, we show that $\SUOT$, $\RSOT$ and $\UOT$ are equivalent under specific conditions on $(\varphi_1, \varphi_2)$, $(\Co, \Cd)$ and $(\al, \be)$. Note that the notion of equivalence we consider here is the same as in \cite[Theorem 2.1.(i)]{bayraktar2019strong}. %

\cb{
\begin{theorem}
    For any $\al,\be\in \Mmp(\mathbb{R}^d)$,
    \begin{equation}
        \SUOT(\al, \be) \le \RSOT(\al,\be).
    \end{equation}
    Moreover, for $p\in [1,\infty)$, $\Co(x,y) = \abs{x-y}^p,\, (x,y) \in \rset^2$ and $\Cd(x,y) = \| x-y \|^p,\, (x,y) \in (\Rd)^2$, for any $\al,\be\in \Mmp(\mathbb{R}^d)$,
    \begin{equation} \label{eq:equiv_loss}
        \SUOT(\al,\be)\leq\RSOT(\al,\be) \leq \UOT(\al,\be) \,.
    \end{equation}
\end{theorem}
\begin{remark}
    \Eqref{eq:equiv_loss} holds provided $\Co\big(\theta^\star(x),\theta^\star(y)\big) \le \Cd(x,y)$.
\end{remark}
\begin{theorem}
    Let $\mathsf{X}$ be a compact subset of $\Rd$ with radius $R$. Consider $\Co(x,y) = \abs{x-y}^p,\, (x,y) \in \rset^2$ and $\Cd(x,y) = \| x-y \|^p,\, (x,y) \in (\Rd)^2$, $p \in [1, +\infty)$. If $D_{\varphi_1} = D_{\varphi_2} = \rho \KL$, or $p=1$ and $\D_{\varphi_1}=\D_{\varphi_2}=\rho\TV$, then for any $\al,\be\in\Mmp(\mathsf{X})$,
    \begin{align*}
        &\UOT(\al,\be) \leq c(m(\al), m(\be), \rho, R)~\SUOT(\al, \be)^{\frac{1}{d+1}} \,,
    \end{align*}
    where $c(m(\al), m(\be), \rho, R)$ is a constant depending on $m(\al), m(\be), \rho, R$, which is non-decreasing in $m(\al)$ and $m(\be)$.
    If $m(\al) \leq M$, $m(\be) \leq M$, then $c(m(\al), m(\be), \rho, R)$ does not depend on $m(\al), m(\be)$, thus $\SUOT$, $\RSOT$ and $\UOT$ are equivalent.
\end{theorem}
}

\begin{theorem}{\textbf{(Equivalence of $\SUOT$, $\RSOT$, $\UOT$)}}
\label{thm:equiv-loss}
    Let $\mathsf{X}$ be a compact subset of $\Rd$ with radius $R$. Consider $\Co(x,y) = \abs{x-y}^p,\, (x,y) \in \rset^2$ and $\Cd(x,y) = \| x-y \|^p,\, (x,y) \in (\Rd)^2$, $p \in [1, +\infty)$. 
    Then, for any $\al, \be \in \Mmp(\mathsf{X})$,
    \begin{align} %
        &\SUOT(\al,\be)\leq\RSOT(\al,\be) \leq \UOT(\al,\be) \,.
    \end{align}
    Additionally, if $D_{\varphi_1} = D_{\varphi_2} = \rho \KL$, or $\Co(x,y)=\abs{x-y}$ and $\D_{\varphi_1}=\D_{\varphi_2}=\rho\TV$, then,
    \begin{align*}
        &\UOT(\al,\be) \leq c(m(\al), m(\be), \rho, R)~\SUOT(\al, \be)^{\frac{1}{d+1}} \,,
    \end{align*}
    where $c(m(\al), m(\be), \rho, R)$ is a constant depending on $m(\al), m(\be), \rho, R$, which is non-decreasing in $m(\al)$ and $m(\be)$.
    If $m(\al) \leq M$, $m(\be) \leq M$, then $c(m(\al), m(\be), \rho, R)$ does not depend on $m(\al), m(\be)$, thus $\SUOT$, $\RSOT$ and $\UOT$ are equivalent.
\end{theorem}

\Cref{thm:equiv-loss} is an application of a more general result, which we derive in \Cref{app:proof-equiv}. In particular, we show that the first two inequalities in \eqref{eq:equiv_loss} hold under milder assumptions on $\varphi_1, \varphi_2$ and $\Co, \Cd$. \textcolor{red}{Je ne comprends pas trop, il me semble que \eqref{eq:equiv_loss} est valable pour tout les $\varphi$ et sur $\mathbb{R}^d$, mais c'est pas ce qui est écrit en appendix ? On peut être plus clair / rescinder en 2 le \Cref{thm:equiv-loss} ?}
The equivalence of $\SUOT, \RSOT$ and $\UOT$ is useful to prove that $\SUOT$ and $\RSOT$ \emph{metrize the weak$^*$ convergence} when $\UOT$ does, e.g. in the GHK setting \cite[Theorem 7.25]{liero2018optimal}.
This result was also unproved for Partial OT, and thus complements contributions of~\citep{bonneel2019spot,bai2022sliced}. %
We recall that a sequence of positive measures $(\alpha_n)_{n \in \nsets}$ converges weakly to $\al\in\Mmp(\rset^d)$ (denoted $\al_n\rightharpoonup\al$) if for any continuous $\f:\Rd\rightarrow\rset$, $\lim_{n \to +\infty} \int\f\rmd\al_n = \int\f\rmd\al$.

\begin{theorem}{\textbf{(Weak$^*$ metrization)}}\label{thm:weak-cv}
Write $\Co(x,y)=\abs{x-y}^p$, $\Cd(x,y)=\|x-y\|^p$ ($p\geq 1$).
Assume either: (i) $\D_{\varphi_1}=\D_{\varphi_2}=\rho\KL$; (ii) $\D_{\varphi_1}=\D_{\varphi_2}=\rho\TV$ and $p=1$. 
Let $(\al_n)$ be a sequence of measures in $\Mmp(\mathsf{X})$ and $\al\in\Mmp(\mathsf{X})$, where $\mathsf{X} \subset \Rd$ is compact with radius $R > 0$. 
Then, $\SUOT$ and $\RSOT$ metrize the weak$^*$ convergence, \ie~
$\al_n\rightharpoonup\al%
\Leftrightarrow \lim_{n\to+\infty} \SUOT(\al_n,\al) = 0 \Leftrightarrow \lim_{n\to+\infty} \RSOT(\al_n,\al) = 0.$
\end{theorem}

The metrization of weak$^*$ convergence is an important property when comparing measures. For instance, it can be leveraged to justify the well-posedness of approximating an unbalanced Wasserstein gradient flow~\citep{ambrosio2005gradient} using $\SUOT$, as done in \citep{candau_tilh, bonet2021sliced} for $\SOT$. Unbalanced Wasserstein gradient flows have been a key tool in deep learning theory, e.g. to prove global convergence of 1-hidden layer neural networks~\citep{chizat2018global,rotskoff2019global}. %





We move on to the statistical properties and prove that $\SUOT$ offers important statistical benefits, as it lifts the \emph{sample complexity} of $\UOT$ from one-dimensional setting to multi-dimensional ones. In what follows, for any $\al \in \Mmp(\Rd)$, we use $\hat{\al}_n$ to denote the empirical approximation of $\al$ over $n \geq 1$ i.i.d. samples, \ie, $\hat{\al}_n = (1/n) \sum_{i=1}^n \updelta_{Z_i}$, $Z_i \sim \al$. 
\begin{theorem}{\textbf{(Sample complexity)}}
\label{thm:sample-comp}
\emph{(i)} If for $\mu,\nu \in\Mmp(\rset)$, $\EE|\UOT(\mu,\nu) -  \UOT(\hat\mu_n,\hat\nu_n)|\leq \kappa(n)$, then for $\al,\be\in\Mmp(\Rd)$, $\EE|\SUOT(\al,\be) -  \SUOT(\hat\al_n,\hat\be_n)|\leq \kappa(n)$. 

\emph{(ii)} If for $\mu \in\Mmp(\rset)$, $\EE|\UOT(\mu,\hat\mu_n)|\leq \xi(n)$, then for $\al \in\Mmp(\Rd)$, $\EE|\SUOT(\al,\hat\al_n)|\leq \xi(n)$.
\end{theorem}

\Cref{thm:sample-comp} shows that $\SUOT$ enjoys a \emph{dimension-free} sample complexity, even when comparing multivariate measures: this advantage is recurrent of sliced divergences \citep{nadjahi2020statistical} and further motivates their use on high-dimensional settings. 
The sample complexity rates $\kappa(n)$ or $\xi(n)$ can be deduced from the $\UOT$ literature on univariate measures for the GHK setting \citep{vacher2022stability}. 

The statistical properties are more challenging to establish for $\RSOT$, since this is not an instance of the general class of sliced divergences introduced in \citep{nadjahi2020statistical}. Therefore, different techniques are needed to derive the sample complexity of $\RSOT$. Inspired by prior work \citep{vacher2022stability}, one promising direction is the analysis of the dual potentials: we leave it for future work.




We conclude this section by deriving the dual formulations of $\SUOT, \RSOT$ and proving that strong duality holds. We will consider that $\unifS$ is approximated with $\hat{\unifS}_K = (1/K) \sum_{k=1}^K\updelta_{\theta_k}$, $\theta_k \sim \unifS$. This corresponds to the routine case in practice, as practitioners usually resort to a Monte Carlo approximation to estimate the expectation w.r.t. $\unifS$ defining sliced OT. 

\begin{theorem}{\textbf{(Strong duality)}}
\label{thm:duality-rsot}
    For $i \in \{1, 2\}$, let $\varphi_i$ be an entropy function s.t. $\dom(\phi_i^*)\cap\rset_{-}$ is non-empty, and either $0\in\dom(\phi_i)$ or $m(\al),m(\be) \in\dom(\phi_i)$.
    Let $\calE\triangleq\{ (f_\theta, g_\theta)_{\theta\in\supp(\sigma_K)}\,:\,\forall \theta\in\supp(\sigma_K), \f_\theta\oplus\g_\theta\leq\Co \}$, $\f_{avg}(x)\triangleq\int_{\sphereD} \f_\theta(x)\rmd\hat{\unifS}_K(\theta)$ and $\g_{avg}(y)\triangleq\int_{\sphereD} \g_\theta(y)\rmd\hat{\unifS}_K(\theta)$. Then, %
    $\SUOT(\al,\be) = \sup_{(\f_\theta),(\g_\theta)\in\calE} \calD_1(\f_\theta,\g_\theta)$ and 
    $\RSOT(\al,\be) = \sup_{(\f_\theta),(\g_\theta)\in\calE} \calD_2(\f_\theta,\g_\theta)$, where
    \begin{align}
        \calD_1(\f_\theta,\g_\theta)&\triangleq
        \int_{\sphereD} \int\phi_1^\circ\big(\f_\theta\circ\theta^\star(x)\big)\rmd\al(x)\rmd\hat{\unifS}_K(\theta)\label{eq:dual-suot}%
        + \int_{\sphereD} \int\phi_2^\circ\big(\g_\theta\circ\theta^\star(y)\big)\rmd\be(y)\rmd\hat{\unifS}_K(\theta)%
        \\
        \calD_2(\f_\theta,\g_\theta)&\triangleq
        \int \phi_1^\circ\big(\f_{avg}\circ\theta^\star(x)\big)\rmd\al(x)\label{eq:dual-rsot}%
        + \int \phi_2^\circ\big(\g_{avg}\circ\theta^\star(y)\big)\rmd\be(y) %
    \end{align} 
\end{theorem}
We conjecture that strong duality also holds for $\unifS$ Lebesgue over $\sphereD$: see \Cref{app:proof-duality}. \Cref{thm:duality-rsot} has important pratical implications, since it justifies the Frank-Wolfe-type algorithms that we develop in \Cref{sec:implem} to compute $\SUOT$ and $\RSOT$ in practice. 

